Proxy2World: Learning to Generate Worlds From Lightweight Proxies without Seeing Them

Lightweight scene proxies let creators control scene layout and motion while leaving room for imagination in appearance, lighting, and visual effects. However, a suitable proxy is not uniquely defined, making paired proxy-video data difficult to construct automatically at scale. We present Proxy2World, a controllable world model that learns these complementary capabilities from ordinary posed RGBD videos, without training on authored proxy-video pairs. The model jointly learns depth-conditioned RGB generation and joint RGBD generation through cross-modal flow matching. Learning both tasks enables proxy-camera hybrid denoising at inference to follow the proxy structure while producing natural, detailed visuals. We further introduce ProxyBench to evaluate this capability across a diverse set of scenes, camera trajectories, and subject motions. Experiments on ProxyBench show that Proxy2World achieves a better balance between structural adherence and visual quality than camera-controlled and geometry-conditioned methods, supported by quantitative metrics, VLM assessments, human evaluations and diverse qualitative results.

==> assets/pairwise-preference.tex <==
% Requires booktabs and graphicx. Frozen snapshot: 2026-09-25T08:39:01.353Z
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{Whitebox adherence: empirical pairwise preference rates. Entries report the percentage preferring the row method over the column method, with ties counted as half a win; comparison counts are in parentheses. This interim snapshot includes valid responses from incomplete sessions.}
\label{tab:user-study-pairwise-adherence}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrr}
\toprule
Row / Column & M1 & M2 & M3 & M4 & M5 & M6 & M7 & M8 & M9 & M10 \\
\midrule
M1 & -- & 77.8\% (9) & 58.3\% (6) & 8.3\% (6) & 8.3\% (6) & 0.0\% (4) & 25.0\% (2) & 0.0\% (8) & 0.0\% (6) & 10.0\% (5) \\
M2 & 22.2\% (9) & -- & 41.7\% (6) & 0.0\% (5) & 0.0\% (6) & 0.0\% (6) & 16.7\% (9) & 0.0\% (6) & 0.0\% (1) & 10.0\% (5) \\
M3 & 41.7\% (6) & 58.3\% (6) & -- & 12.5\% (8) & 0.0\% (7) & 0.0\% (3) & 25.0\% (8) & 14.3\% (7) & 8.3\% (6) & 0.0\% (6) \\
M4 & 91.7\% (6) & 100.0\% (5) & 87.5\% (8) & -- & 7.1\% (7) & 25.0\% (4) & 43.8\% (8) & 12.5\% (8) & 17.9\% (14) & 30.0\% (5) \\
M5 & 91.7\% (6) & 100.0\% (6) & 100.0\% (7) & 92.9\% (7) & -- & 41.7\% (6) & 66.7\% (3) & 50.0\% (8) & 58.3\% (6) & 40.0\% (5) \\
M6 & 100.0\% (4) & 100.0\% (6) & 100.0\% (3) & 75.0\% (4) & 58.3\% (6) & -- & 83.3\% (6) & 66.7\% (3) & 100.0\% (6) & 58.3\% (6) \\
M7 & 75.0\% (2) & 83.3\% (9) & 75.0\% (8) & 56.3\% (8) & 33.3\% (3) & 16.7\% (6) & -- & 0.0\% (5) & 0.0\% (5) & 10.0\% (5) \\
M8 & 100.0\% (8) & 100.0\% (6) & 85.7\% (7) & 87.5\% (8) & 50.0\% (8) & 33.3\% (3) & 100.0\% (5) & -- & 50.0\% (8) & 50.0\% (5) \\
M9 & 100.0\% (6) & 100.0\% (1) & 91.7\% (6) & 82.1\% (14) & 41.7\% (6) & 0.0\% (6) & 100.0\% (5) & 50.0\% (8) & -- & 75.0\% (6) \\
M10 & 90.0\% (5) & 90.0\% (5) & 100.0\% (6) & 70.0\% (5) & 60.0\% (5) & 41.7\% (6) & 90.0\% (5) & 50.0\% (5) & 25.0\% (6) & -- \\
\bottomrule
\end{tabular}%
}
\par\smallskip
\begin{minipage}{\textwidth}\scriptsize
M1: RAYPE; M2: Lyra2; M3: FantasyWorld; M4: Ours CAM-TI2V; M5: Cosmos-Depth; M6: VACE-Depth; M7: C2R; M8: Ours T2V $P=P^*$; M9: Ours TI2V $P=P^*$; M10: Ours T2V $P=0$ (depth40).
\end{minipage}
\end{table*}

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{Refinement: empirical pairwise preference rates. Entries report the percentage preferring the row method over the column method, with ties counted as half a win; comparison counts are in parentheses. This interim snapshot includes valid responses from incomplete sessions.}
\label{tab:user-study-pairwise-refinement}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrr}
\toprule
Row / Column & M1 & M2 & M3 & M4 & M5 & M6 & M7 & M8 & M9 & M10 \\
\midrule
M1 & -- & 83.3\% (6) & 25.0\% (4) & 16.7\% (9) & 16.7\% (6) & 37.5\% (8) & 28.6\% (7) & 0.0\% (4) & 0.0\% (4) & 66.7\% (3) \\
M2 & 16.7\% (6) & -- & 50.0\% (6) & 11.1\% (9) & 0.0\% (6) & 0.0\% (2) & 62.5\% (4) & 0.0\% (6) & 0.0\% (9) & 50.0\% (4) \\
M3 & 75.0\% (4) & 50.0\% (6) & -- & 25.0\% (6) & 0.0\% (8) & 14.3\% (7) & 42.9\% (7) & 0.0\% (3) & 0.0\% (7) & 16.7\% (3) \\
M4 & 83.3\% (9) & 88.9\% (9) & 75.0\% (6) & -- & 75.0\% (8) & 83.3\% (6) & 70.0\% (5) & 40.0\% (5) & 0.0\% (2) & 58.3\% (6) \\
M5 & 83.3\% (6) & 100.0\% (6) & 100.0\% (8) & 25.0\% (8) & -- & 42.9\% (7) & 91.7\% (6) & 8.3\% (6) & 25.0\% (4) & 66.7\% (3) \\
M6 & 62.5\% (8) & 100.0\% (2) & 85.7\% (7) & 16.7\% (6) & 57.1\% (7) & -- & 20.0\% (5) & 0.0\% (7) & 20.0\% (5) & 66.7\% (3) \\
M7 & 71.4\% (7) & 37.5\% (4) & 57.1\% (7) & 30.0\% (5) & 8.3\% (6) & 80.0\% (5) & -- & 0.0\% (10) & 7.1\% (7) & 30.0\% (5) \\
M8 & 100.0\% (4) & 100.0\% (6) & 100.0\% (3) & 60.0\% (5) & 91.7\% (6) & 100.0\% (7) & 100.0\% (10) & -- & 40.0\% (5) & 90.0\% (5) \\
M9 & 100.0\% (4) & 100.0\% (9) & 100.0\% (7) & 100.0\% (2) & 75.0\% (4) & 80.0\% (5) & 92.9\% (7) & 60.0\% (5) & -- & 100.0\% (4) \\
M10 & 33.3\% (3) & 50.0\% (4) & 83.3\% (3) & 41.7\% (6) & 33.3\% (3) & 33.3\% (3) & 70.0\% (5) & 10.0\% (5) & 0.0\% (4) & -- \\
\bottomrule
\end{tabular}%
}
\par\smallskip
\begin{minipage}{\textwidth}\scriptsize
M1: RAYPE; M2: Lyra2; M3: FantasyWorld; M4: Ours CAM-TI2V; M5: Cosmos-Depth; M6: VACE-Depth; M7: C2R; M8: Ours T2V $P=P^*$; M9: Ours TI2V $P=P^*$; M10: Ours T2V $P=0$ (depth40).
\end{minipage}
\end{table*}

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{Overall preference: empirical pairwise preference rates. Entries report the percentage preferring the row method over the column method, with ties counted as half a win; comparison counts are in parentheses. This interim snapshot includes valid responses from incomplete sessions.}
\label{tab:user-study-pairwise-overall}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrr}
\toprule
Row / Column & M1 & M2 & M3 & M4 & M5 & M6 & M7 & M8 & M9 & M10 \\
\midrule
M1 & -- & 50.0\% (4) & 31.3\% (8) & 0.0\% (3) & 0.0\% (6) & 16.7\% (6) & 55.6\% (9) & 0.0\% (6) & 0.0\% (8) & 0.0\% (2) \\
M2 & 50.0\% (4) & -- & 42.9\% (7) & 0.0\% (4) & 0.0\% (6) & 5.0\% (10) & 0.0\% (5) & 0.0\% (6) & 0.0\% (8) & 0.0\% (3) \\
M3 & 68.8\% (8) & 57.1\% (7) & -- & 12.5\% (4) & 0.0\% (4) & 25.0\% (8) & 66.7\% (3) & 12.5\% (8) & 20.0\% (5) & 0.0\% (3) \\
M4 & 100.0\% (3) & 100.0\% (4) & 87.5\% (4) & -- & 25.0\% (4) & 37.5\% (8) & 83.3\% (6) & 10.0\% (5) & 0.0\% (2) & 100.0\% (2) \\
M5 & 100.0\% (6) & 100.0\% (6) & 100.0\% (4) & 75.0\% (4) & -- & 40.0\% (5) & 77.8\% (9) & 37.5\% (4) & 31.3\% (8) & 100.0\% (3) \\
M6 & 83.3\% (6) & 95.0\% (10) & 75.0\% (8) & 62.5\% (8) & 60.0\% (5) & -- & 100.0\% (7) & 37.5\% (8) & 25.0\% (8) & 33.3\% (3) \\
M7 & 44.4\% (9) & 100.0\% (5) & 33.3\% (3) & 16.7\% (6) & 22.2\% (9) & 0.0\% (7) & -- & 0.0\% (3) & 0.0\% (6) & 25.0\% (2) \\
M8 & 100.0\% (6) & 100.0\% (6) & 87.5\% (8) & 90.0\% (5) & 62.5\% (4) & 62.5\% (8) & 100.0\% (3) & -- & 50.0\% (5) & 100.0\% (3) \\
M9 & 100.0\% (8) & 100.0\% (8) & 80.0\% (5) & 100.0\% (2) & 68.8\% (8) & 75.0\% (8) & 100.0\% (6) & 50.0\% (5) & -- & 100.0\% (3) \\
M10 & 100.0\% (2) & 100.0\% (3) & 100.0\% (3) & 0.0\% (2) & 0.0\% (3) & 66.7\% (3) & 75.0\% (2) & 0.0\% (3) & 0.0\% (3) & -- \\
\bottomrule
\end{tabular}%
}
\par\smallskip
\begin{minipage}{\textwidth}\scriptsize
M1: RAYPE; M2: Lyra2; M3: FantasyWorld; M4: Ours CAM-TI2V; M5: Cosmos-Depth; M6: VACE-Depth; M7: C2R; M8: Ours T2V $P=P^*$; M9: Ours TI2V $P=P^*$; M10: Ours T2V $P=0$ (depth40).
\end{minipage}
\end{table*}



==> assets/preference-table.tex <==
% Snapshot 2026-09-25T08:39:01.353Z; tie-adjusted empirical preference rates, not BT scores. Requires booktabs.
\begin{tabular}{lrrr}
\toprule
Method & Adherence & Refinement & Overall \\
\midrule
RAYPE & 24.0\% (52) & 30.4\% (51) & 20.2\% (52) \\
Lyra2 & 12.3\% (53) & 18.3\% (52) & 10.4\% (53) \\
FantasyWorld & 18.4\% (57) & 23.5\% (51) & 32.0\% (50) \\
Ours CAM-TI2V & 42.3\% (65) & 71.4\% (56) & 57.9\% (38) \\
Cosmos-Depth & 72.2\% (54) & 61.1\% (54) & 71.4\% (49) \\
VACE-Depth & 81.8\% (44) & 44.0\% (50) & 65.9\% (63) \\
C2R & 43.1\% (51) & 33.0\% (56) & 27.0\% (50) \\
Ours T2V $P=P^*$ & 75.0\% (58) & 88.2\% (51) & 82.3\% (48) \\
Ours TI2V $P=P^*$ & 69.0\% (58) & 90.4\% (47) & 84.9\% (53) \\
Ours T2V $P=0$ & 67.7\% (48) & 38.9\% (36) & 47.9\% (24) \\
\bottomrule
\end{tabular}

